FairTune: Optimizing Parameter Efficient Fine Tuning for Fairness in Medical Image Analysis

Training models with robust group fairness properties is crucial in ethically sensitive application areas such as medical diagnosis. Despite the growing body of work aiming to minimise demographic bias in AI, this problem remains challenging. A key reason for this challenge is the fairness generalisation gap: High-capacity deep learning models can fit all training data nearly perfectly, and thus also exhibit perfect fairness during training. In this case, bias emerges only during testing when generalisation performance differs across subgroups. This motivates us to take a bi-level optimisation perspective on fair learning: Optimising the learning strategy based on validation fairness. Specifically, we consider the highly effective workflow of adapting pre-trained models to downstream medical imaging tasks using parameter-efficient fine-tuning (PEFT) techniques. There is a trade-off between updating more parameters, enabling a better fit to the task of interest vs. fewer parameters, potentially reducing the generalisation gap. To manage this tradeoff, we propose FairTune, a framework to optimise the choice of PEFT parameters with respect to fairness. We demonstrate empirically that FairTune leads to improved fairness on a range of medical imaging datasets. The code is available at https://github.com/Raman1121/FairTune

==> tables/HAM10000_age_distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llll@{}}
        & Label 0 & Label 1 & Split                       \\
Group 0 & 5218    & 545     & \multirow{2}{*}{Train}      \\
Group 1 & 1618    & 586     &                             \\
        &         &         &                             \\
Group 0 & 604     & 69      & \multirow{2}{*}{Validation} \\
Group 1 & 219     & 97      &                             \\
        &         &         &                             \\
Group 0 & 653     & 70      & \multirow{2}{*}{Test}       \\
Group 1 & 208     & 71      &                            
\end{tabular}
\end{table}

==> tables/HAM10K_GENDER_distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llll@{}}
       & Label 0 & Label 1 & Split                                     \\
Male   & 3609    & 725     & \multirow{2}{*}{Train}                    \\
Female & 3224    & 406     &                                           \\
       &         &         &                                           \\
Male   & 419     & 104     & \multirow{2}{*}{Validation}               \\
Female & 399     & 62      &                                           \\
       &         &         &                                           \\
Male   & 464     & 79      & \multicolumn{1}{c}{\multirow{2}{*}{Test}} \\
Female & 395     & 62      & \multicolumn{1}{c}{}                     
\end{tabular}
\end{table}

==> tables/OASIS_Age_distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
        & Label 0 & Label 1 & Split                       \\
Group 0 & 3836    & 1768    & \multirow{2}{*}{Train}      \\
Group 1 & 1716    & 2392    &                             \\
        &         &         &                             \\
Group 0 & 468     & 312     & \multirow{2}{*}{Validation} \\
Group 1 & 312     & 104     &                             \\
        &         &         &                             \\
Group 0 & 364     & 260     & \multirow{2}{*}{Test}       \\
Group 1 & 260     & 364     &                            
\end{tabular}
\end{table}

==> tables/OASIS_Gender_Distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
       & Label 0 & Label 1 & Split                       \\
Male   & 1476    & 1924    & \multirow{2}{*}{Train}      \\
Female & 4076    & 2236    &                             \\
       &         &         &                             \\
Male   & 208     & 104     & \multirow{2}{*}{Validation} \\
Female & 572     & 312     &                             \\
       &         &         &                             \\
Male   & 260     & 104     & \multirow{2}{*}{Test}       \\
Female & 364     & 520     &                            
\end{tabular}
\end{table}

==> tables/OL3I_Age_Distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
        & Label 0 & Label 1 & Split                       \\
Group 0 & 3512    & 87      & \multirow{2}{*}{Train}      \\
Group 1 & 1487    & 141     &                             \\
        &         &         &                             \\
Group 0 & 830     & 13      & \multirow{2}{*}{Validation} \\
Group 1 & 417     & 43      &                             \\
        &         &         &                             \\
Group 0 & 1060    & 25      & \multirow{2}{*}{Test}       \\
Group 1 & 478     & 46      &                            
\end{tabular}
\end{table}

==> tables/OL3I_Gender_distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
       & Label 0 & Label 1 & Split                       \\
Male   & 1984    & 111     & \multirow{2}{*}{Train}      \\
Female & 3015    & 117     &                             \\
       &         &         &                             \\
Male   & 498     & 32      & \multirow{2}{*}{Validation} \\
Female & 749     & 24      &                             \\
       &         &         &                             \\
Male   & 629     & 39      & \multirow{2}{*}{Test}       \\
Female & 909     & 32      &                            
\end{tabular}
\end{table}

==> tables/PAPILA_AGE_Distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
        & Label 0 & Label 1 & Split                       \\
Group 0 & 117     & 9       & \multirow{2}{*}{Train}      \\
Group 1 & 123     & 45      &                             \\
        &         &         &                             \\
Group 0 & 18      & 2       & \multirow{2}{*}{Validation} \\
Group 1 & 11      & 11      &                             \\
        &         &         &                             \\
Group 0 & 28      & 4       & \multirow{2}{*}{Test}       \\
Group 1 & 36      & 16      &                            
\end{tabular}
\end{table}

==> tables/PAPILA_Gender_Distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llll@{}}
       & Label 0 & Label 1 & Split                       \\
Male   & 70      & 18      & \multirow{2}{*}{Train}      \\
Female & 170     & 36      &                             \\
       &         &         &                             \\
Male   & 13      & 9       & \multirow{2}{*}{Validation} \\
Female & 16      & 4       &                             \\
       &         &         &                             \\
Male   & 28      & 8       & \multirow{2}{*}{Test}       \\
Female & 36      & 12      &                            
\end{tabular}
\end{table}

==> tables/all_datasets_info.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}llll@{}}
\toprule
Dataset        & Modality                        & Size  & Sensitive Attribute \\ \midrule
PAPILA         & Fundus Image (2D)               & 420   & Age, Sex            \\
OL3I           & Heart CT (2D)                   & 8139  & Age, Sex            \\
HAM10000       & Skin Dermatology (2D)           & 9948  & Age, Sex            \\
OASIS          & Brain MRI (3D -\textgreater 2D) & 12156 & Age, Sex            \\
Fitzpatrick17K & Skin Dermatology (2D)           & 16012 & Skin Type          
\end{tabular}
\end{table}

==> tables/cosine_sim_hamming_dist.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lllrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Sensitive Attribute}} & \multicolumn{1}{c}{\textbf{Tuning Method}} & \multicolumn{1}{c}{\textbf{Cosine Similarity}} & \multicolumn{1}{c}{\textbf{Hamming Distance}} \\ \midrule
                                     &                                                  &                                            & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\
Fitzpatrick                          & Skin\_type                                       & Tune Full Block                            & 0.500                                          & 0.500                                         \\
Fitzpatrick                          & Skin\_type                                       & Tune Attention                             & 0.447                                          & 0.417                                         \\
Fitzpatrick                          & Skin\_type                                       & Tune LayerNorm                             & 0.632                                          & 0.417                                         \\
Fitzpatrick                          & Skin\_type                                       & AutoPEFT                                   & 0.450                                          & 0.611                                         \\
                                     &                                                  &                                            & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\
HAM10000                             & Age                                              & Tune Full Block                            & 0.612                                          & 0.417                                         \\
HAM10000                             & Age                                              & Tune Attention                             & 0.707                                          & 0.250                                         \\
HAM10000                             & Age                                              & Tune LayerNorm                             & 0.566                                          & 0.583                                         \\
HAM10000                             & Age                                              & AutoPEFT                                   & 0.579                                          & 0.528                                         \\
HAM10000                             & Gender                                           & Tune Full Block                            & 0.378                                          & 0.583                                         \\
HAM10000                             & Gender                                           & Tune Attention                             & 0.507                                          & 0.500                                         \\
HAM10000                             & Gender                                           & Tune LayerNorm                             & 0.316                                          & 0.750                                         \\
HAM10000                             & Gender                                           & AutoPEFT                                   & 0.620                                          & 0.444                                         \\
                                     &                                                  &                                            & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\
papila                               & Age                                              & Tune Full Block                            & 0.474                                          & 0.583                                         \\
papila                               & Age                                              & Tune Attention                             & 0.617                                          & 0.417                                         \\
papila                               & Age                                              & Tune LayerNorm                             & 0.802                                          & 0.250                                         \\
papila                               & Age                                              & AutoPEFT                                   & 0.501                                          & 0.444                                         \\
papila                               & Gender                                           & Tune Full Block                            & 0.474                                          & 0.583                                         \\
papila                               & Gender                                           & Tune Attention                             & 0.676                                          & 0.333                                         \\
papila                               & Gender                                           & Tune LayerNorm                             & 0.400                                          & 0.500                                         \\
papila                               & Gender                                           & AutoPEFT                                   & 0.400                                          & 0.667                                         \\
                                     &                                                  &                                            & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\
ol3i                                 & Age                                              & Tune Full Block                            & 0.250                                          & 0.500                                         \\
ol3i                                 & Age                                              & Tune Attention                             & 0.189                                          & 0.750                                         \\
ol3i                                 & Age                                              & Tune LayerNorm                             & 0.667                                          & 0.500                                         \\
ol3i                                 & Age                                              & AutoPEFT                                   & 0.520                                          & 0.472                                         \\
ol3i                                 & Gender                                           & Tune Full Block                            & 0.571                                          & 0.500                                         \\
ol3i                                 & Gender                                           & Tune Attention                             & 0.436                                          & 0.500                                         \\
ol3i                                 & Gender                                           & Tune LayerNorm                             & 0.309                                          & 0.750                                         \\
ol3i                                 & Gender                                           & AutoPEFT                                   & 0.653                                          & 0.389                                         \\
                                     &                                                  &                                            & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\
oasis                                & Age                                              & Tune Full Block                            & 0.333                                          & 0.667                                         \\
oasis                                & Age                                              & Tune Attention                             & 0                                              & 1                                             \\
oasis                                & Age                                              & Tune LayerNorm                             & 0.617                                          & 0.417                                         \\
oasis                                & Age                                              & AutoPEFT                                   & 0.415                                          & 0.500                                         \\
oasis                                & Age                                              & auto\_peft1                                & 0.415                                          & 0.500                                         \\ \bottomrule
\end{tabular}
\end{table}

==> tables/fitzpatrick_distribution.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llll@{}}
\toprule
        & Label 0 & Label 1 & Split                                      \\ \midrule
Group 0 & 7538    & 1312    & \multicolumn{1}{c}{\multirow{2}{*}{Train}} \\
Group 1 & 3541    & 418     & \multicolumn{1}{c}{}                       \\
        &         &         &                                            \\
Group 0 & 940     & 159     & \multirow{2}{*}{Validation}                \\
Group 1 & 456     & 46      &                                            \\
        &         &         &                                            \\
Group 0 & 934     & 180     & \multicolumn{1}{c}{\multirow{2}{*}{Test}}  \\
Group 1 & 443     & 45      & \multicolumn{1}{c}{}                       \\ \cmidrule(r){1-3}
\end{tabular}
\end{table}

==> tables/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llllllllllllll@{}}
\toprule
Dataset         & Sensitive Attribute & Full FT & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Linear \\ Readout\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Block Tuning\\ (Vanilla)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Block Tuning\\ (Obj: Overall AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Block Tuning\\ (Obj: Min AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Attention Tuning\\ (Vanilla)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Attention Tuning\\ (Obj: Overall AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}LayerNorm Tuning\\ (Vanilla)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}LayerNorm Tuning\\ (Obj: Overall AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}LayerNorm Tuning\\ (Obj: Min AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}AutoPEFT\\ (Obj: Overall AUC)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}AutoPEFT\\ (Obj: Min AUC)\end{tabular}} \\ \midrule
Fitzpatrick 17K & Skin Type           &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                &                     &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
HAM10000        & Age                 &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                & Gender              &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                &                     &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
PAPILA          & Age                 &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                & Gender              &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                &                     &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
OL3I            & Age                 &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                & Gender              &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                &                     &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
Oasis           & Age                 &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                & Gender              &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\
                &                     &         &                                                                               &                                                                                      &                                                                                               &                                                                                           &                                                                                          &                                                                                                   &                                                                                          &                                                                                                   &                                                                                               &                                                                                           &                                                                                       \\ \bottomrule
\end{tabular}
}
\end{table}
